Document-level Entity-based Extraction as Template Generation

Document-level entity-based extraction (EE), aiming at extracting entity-centric information such as entity roles and entity relations, is key to automatic knowledge acquisition from text corpora for various domains. Most document-level EE systems build extractive models, which struggle to model long-term dependencies among entities at the document level. To address this issue, we propose a generative framework for two document-level EE tasks: role-filler entity extraction (REE) and relation extraction (RE). We first formulate them as a template generation problem, allowing models to efficiently capture cross-entity dependencies, exploit label semantics, and avoid the exponential computation complexity of identifying N-ary relations. A novel cross-attention guided copy mechanism, TopK Copy, is incorporated into a pre-trained sequence-to-sequence model to enhance the capabilities of identifying key information in the input document. Experiments done on the MUC-4 and SciREX dataset show new state-of-the-art results on REE (+3.26%), binary RE (+4.8%), and 4-ary RE (+2.7%) in F1 score.

==> tables/dataset_stats.tex <==
\begin{table*}[t]
    \small
    \centering
    {
    \begin{tabular}{lccccccccc}
        \toprule
        
        & \multicolumn{3}{c}{\textbf{Role-filler Entity Extraction}} & 
        
        \midrule
        \multirow{3}{*}{MUC-4 REE} & Train \\
         & Dev \\
         & Test \\
        \\
        % SciREX BRE \\
        % SciREX 4RE \\
        
        

        
        
        \bottomrule
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{Data statistics of MUC-4 and SciREX.}
    \label{tab:ablation}
    
\end{table*}
